ChewBaccaNN: A Flexible 223 TOPS/W BNN Accelerator

Binary Neural Networks enable smart IoT devices, as they significantly reduce the required memory footprint and computational complexity while retaining a high network performance and flexibility. This paper presents ChewBaccaNN, a 0.7 mm$^2$ sized binary convolutional neural network (CNN) accelerator designed in GlobalFoundries 22 nm technology. By exploiting efficient data re-use, data buffering, latch-based memories, and voltage scaling, a throughput of 241 GOPS is achieved while consuming just 1.1 mW at 0.4V/154MHz during inference of binary CNNs with up to 7x7 kernels, leading to a peak core energy efficiency of 223 TOPS/W. ChewBaccaNN's flexibility allows to run a much wider range of binary CNNs than other accelerators, drastically improving the accuracy-energy trade-off beyond what can be captured by the TOPS/W metric. In fact, it can perform CIFAR-10 inference at 86.8% accuracy with merely 1.3 $\mu J$, thus exceeding the accuracy while at the same time lowering the energy cost by 2.8x compared to even the most efficient and much larger analog processing-in-memory devices, while keeping the flexibility of running larger CNNs for higher accuracy when needed. It also runs a binary ResNet-18 trained on the 1000-class ILSVRC dataset and improves the energy efficiency by 4.4x over accelerators of similar flexibility. Furthermore, it can perform inference on a binarized ResNet-18 trained with 8-bases Group-Net to achieve a 67.5% Top-1 accuracy with only 3.0 mJ/frame -- at an accuracy drop of merely 1.8% from the full-precision ResNet-18.

==> plots/throughputtable.tex <==
technology throughput eneff syntperiod
8202428	591.136	121.921	0
% 770015	186.667	215.096	1.5
770040	39.680	107.300	4
770040	146.542	213.373	4
770040	166.809	208.665	4
% 770080	39.200	102.964	8
770080	78.400	160.985	8
% 770080	130.667	197.009	8
% 770080	104.533	166.734	8
% 770020	130.667	187.736	2
% 770020	156.800	188.116	2
770020	104.533	183.752	2
% 770015	156.800	206.930	1.5
770015	186.667	219.202	1.5
770015	305.237	182.231	1.5
770015	209.067	223.021	1.5
770015	224.000	223.093	1.5
770015	261.333	213.254	1.5
770015	285.091	211.993	1.5
770015	241.231	223.149	1.5
% 770040	196.000	199.941	4
770040	130.667	202.695	4
% 770040	104.533	170.250	4
% 550015	95.238	120.580	1.5
550040	20.245	59.899	4
550040	74.766	117.987	4
550040	85.106	114.920	4
% 550080	20.000	57.391	8
550080	40.000	88.671	8
% 550080	66.667	108.515	8
% 550080	53.333	91.987	8
% 550020	66.667	104.648	2
% 550020	80.000	104.993	2
550020	53.333	101.710	2
% 550015	80.000	115.024	1.5
550015	95.238	120.848	1.5
550015	155.733	100.427	1.5
550015	106.667	123.241	1.5
550015	114.286	124.530	1.5
550015	133.333	119.225	1.5
550015	145.455	117.619	1.5
550015	123.077	124.365	1.5
% 550040	100.000	111.391	4
550040	66.667	112.109	4
% 550040	53.333	94.316	4
% 330015	34.286	62.629	1.5
330040	7.288	31.545	4
330040	26.916	62.625	4
330040	30.638	61.040	4
% 330080	7.200	29.884	8
330080	14.400	46.778	8
% 330080	24.000	57.239	8
% 330080	19.200	48.909	8
% 330020	24.000	54.420	2
% 330020	28.800	54.711	2
330020	19.200	53.093	2
% 330015	28.800	60.632	1.5
330015	34.286	63.290	1.5
330015	56.064	52.755	1.5
330015	38.400	65.375	1.5
330015	41.143	65.315	1.5
330015	48.000	62.339	1.5
330015	52.364	61.291	1.5
330015	44.308	65.273	1.5
% 330040	36.000	58.798	4
330040	24.000	59.600	4
% 330040	19.200	50.000	4
